Fusing Odometry, UWB Ranging, and Spatial Detections for Relative Multi-Robot Localization

This letter presents a cooperative relative multi-robot localization design and experimental study. We propose a flexible Monte Carlo approach leveraging a particle filter to estimate relative states. The estimation can be based on inter-robot Ultra-Wideband (UWB) ranging and onboard odometry alone or dynamically integrated with cooperative spatial object detections from stereo cameras mounted on each robot. The main contributions of this work are as follows. First, we show that a single UWB range is enough to estimate the accurate relative states of two robots when fusing odometry measurements. Second, our experiments also demonstrate that our approach surpasses traditional methods, namely, multilateration, in terms of accuracy. Third, to further increase accuracy, we allow for the integration of cooperative spatial detections. Finally, we show how ROS 2 and Zenoh can be integrated to build a scalable wireless communication solution for multi-robot systems. The experimental validation includes real-time deployment and autonomous navigation based on the relative positioning method. It is worth mentioning that we also address the challenges for UWB-ranging error mitigation for mobile transceivers. The code is available at https://github.com/TIERS/uwb-cooperative-mrs-localization.

==> algs/pf_relative.tex <==
\begin{algorithm}[t]
    \footnotesize
	\caption{Multi-robot relative state estimation.} 
	\label{alg:pf_estimation}
    % \begin{algorithmic}[1]
    \SetAlgoLined
    	Assuming there are $n$ number of robots:
    	$ i \in (1 \sim n) $; 
    	$ j \in (1 \sim n) $; \\
    	Robot or UWB pair: 
    	$ p_{i,j}$;\\
            Particles: $\mathcal{PT}$ \\
    	\KwIn{ \\
    	    \vspace{.42em}
    	    \hspace{1em}UWB range between the pair $p_{i,j}$:  $\mathcal{UR}_{p_{i,j}} $; \\
    	    \vspace{.23em}
    	    \hspace{1em}Random spatial detection information (detected object poses relative to 
         cameras) of robot $p_{i,j}$ (if there are objects detected):  $\mathcal{SD}_{p_{i,j}}$; \\
    	    \vspace{.23em}
    	    \hspace{1em}Odometry data of the robot $i$: $\mathcal{O}_{i}$;\\
    	    \vspace{.23em}
    	}
    	\KwOut{  \\
    	    \vspace{.42em}
    	    \hspace{1em}State estimations of robots: $\textbf{\mathcal{S}}_{i} \leftarrow ({x}_{i}, {y}_{i}), i \in (1 \sim n)$ \\
    	}  
    	\BlankLine 
    	\While{new $\mathcal{UR}_{p_{i,j}}$}{
    	    \vspace{.23em}
    	    UWB ranging error: $URE_{p_{i,j}} \leftarrow stactedLSTM (\mathcal{UR}_{p_{i,j}})$ \\
    	    Corrected UWB ranges: $CUR_{p_{i,j}} \leftarrow \mathcal{UR}_{p_{i,j}} - URE_{p_{i,j}} $\\
    	    At $t=0$, initialize particles $\mathcal{PT}$ based on $\mathcal{O}_{i}$ at time $t=0$ \\ with a  Gaussian distribution  
    	    % 
    	    \If{$\mathcal{PT}$ was initialized}
    	    {
    	        Calculate the movements of $\mathcal{PT}$ based on the $\mathcal{O}_{i}$; \\
    	        \If{number of $\mathcal{SD}_{p_{i,j}}$ \textgreater $0$}
    	        {
    	            \For{All detection pairs from  $\mathcal{SD}_{p_{i,j}}$}
    	            {
    	                The relative vector between robots: \\
                        $ \mathcal{R}_{p_{i,j}}\leftarrow \mathcal{SD}_{p_{i}} - \mathcal{SD}_{p_{j}} $ ; \\
    	                $\mathcal{D}_{p_{i,j}} \leftarrow \lvert \mathcal{R}_{p_{i,j}} \rvert$;\\
    	                \If{$|\mathcal{D}_{p_{i,j}} - \mathcal{CUR}_{p_{i,j}}|$ \textless $d_{th}$}
    	                {
    	                    \tcc{Shared spatial detection;}
    	                    $new\_meas \leftarrow \mathcal{CUR}_{p_{i,j}} , \mathcal{R}_{p_{i,j}} $;
    	                }
    	                % {
    	                %     % \textit{pass}
    	                % }
    	            }
    	        }
    	        {
    	            $new\_meas \leftarrow \mathcal{CUR}_{p_{i,j}} $
    	        }
    	        \textbf{Update filter}\\                 
    	            \hspace{2em} feed $new\_meas$;\\
    	            \hspace{2em} update hypothesis of $\mathcal{PT}$;\\
    	            \hspace{2em} update weights based one $new\_meas$;\\
    	            \hspace{2em} update $\mathcal{PT}$; \\
    	            \hspace{2em} Calculate mean values among $\mathcal{PT}$ to be the $\textbf{\mathcal{S}}_{i}$;
    	   }
        }
\end{algorithm}

==> algs/pf_relative_bak.tex <==
\begin{algorithm}[t]
    \footnotesize
	\caption{Multi-robot relative state estimation.} 
	\label{alg:pf_estimation}
    % \begin{algorithmic}[1]
    \SetAlgoLined
    	Assuming there are $n$ number of robots:
    	$ i \in (1 \sim n) $; 
    	$ j \in (1 \sim n) $; \\
    	Robot or UWB pair: 
    	$ p_{i,j}$;\\
            Particles: $\mathcal{PT}$ \\
    	\KwIn{ \\
    	    \vspace{.42em}
    	    \hspace{1em}UWB range between the pair $p_{i,j}$:  $\mathcal{UR}_{p_{i,j}} $; \\
    	    \vspace{.23em}
    	    \hspace{1em}Random spatial detection information (detected object poses relative to 
         cameras) of robot $p_{i,j}$ (if there are objects detected):  $\mathcal{SD}_{p_{i,j}}$; \\
    	    \vspace{.23em}
    	    \hspace{1em}Odometry data of the robot $i$: $\mathcal{O}_{i}$;\\
    	    \vspace{.23em}
    	}
    	\KwOut{  \\
    	    \vspace{.42em}
    	    \hspace{1em}State estimations of robots: $\textbf{\mathcal{S}}_{i} \leftarrow ({x}_{i}, {y}_{i}), i \in (1 \sim n)$ \\
    	}  
    	\BlankLine 
    	\While{new $\mathcal{UR}_{p_{i,j}}$}{
    	    \vspace{.23em}
    	    UWB ranging error: $URE_{p_{i,j}} \leftarrow stactedLSTM (\mathcal{UR}_{p_{i,j}})$ \\
    	    Corrected UWB ranges: $CUR_{p_{i,j}} \leftarrow \mathcal{UR}_{p_{i,j}} - URE_{p_{i,j}} $\\
    	    At $t=0$, initialize particles $\mathcal{PT}$ based on $\mathcal{O}_{i}$ at time $t=0$ \\ with a  Gaussian distribution  
    	    
    	    \eIf{$\mathcal{PT}$ was initialized}
    	    {
    	        Calculate the movements of $\mathcal{PT}$ based on the $\mathcal{O}_{i}$; \\
    	        \eIf{number of $\mathcal{SD}_{p_{i,j}}$ \textgreater $0$}
    	        {
    	            \For{All detection pairs from  $\mathcal{SD}_{p_{i,j}}$}
    	            {
    	                The relative vector between robots: \\
                        $ \mathcal{R}_{p_{i,j}}\leftarrow \mathcal{SD}_{p_{i}} - \mathcal{SD}_{p_{j}} $ ; \\
    	                $\mathcal{D}_{p_{i,j}} \leftarrow \lvert \mathcal{R}_{p_{i,j}} \rvert$;\\
    	                \eIf{$|\mathcal{D}_{p_{i,j}} - \mathcal{CUR}_{p_{i,j}}|$ \textless $d_{th}$}
    	                {
    	                    \tcc{Shared spatial detection;}
    	                    $new\_meas \leftarrow \mathcal{CUR}_{p_{i,j}} , \mathcal{R}_{p_{i,j}} $;
    	                }
    	                % {
    	                %     % \textit{pass}
    	                % }
    	            }
    	        }
    	        {
    	            $new\_meas \leftarrow \mathcal{CUR}_{p_{i,j}} $
    	        }
    	        \textbf{Update filter}\\                 
    	            \hspace{2em} feed $new\_meas$;\\
    	            \hspace{2em} update hypothesis of $\mathcal{PT}$;\\
    	            \hspace{2em} update weights based one $new\_meas$;\\
    	            \hspace{2em} update $\mathcal{PT}$; \\
    	            \hspace{2em} Calculate mean values among $\mathcal{PT}$ to be the $\textbf{\mathcal{S}}_{i}$;
    	   }
    	    % { 
    	    %    % pass
         %  }
    
    	   % Stop updating $\mathcal{PT}$ if there is no new $\mathcal{UR}_{p_{i,j}}$;
            % \EndWhile
    	   % \vspace{.23em}
    	}
    % \end{algorithmic}
\end{algorithm}

==> sec/03_Methods_old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                          %%
%%              METHODOLOGY                 %%
%%                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Methodology}\label{sec:methodology}

%This section presents details of the multi-robot system for which we design and develop a novel Monte-Carlo cooperative localization method.

Through this section, we introduce the relative localization problem, formulated as an optimization problem with inputs representing inter-robot UWB ranging measurements, individual odometry measurements and cooperative spatial detections. These inputs are conceptually depicted in Fig.~\ref{fig:pf_diagram}, while the summarized localization process is described in Algorithm~\ref{alg:pf_estimation}.

\subsection{Problem Statement} %Multi-Robot 

We use the following notation for the remaining of this paper. We consider a group of $N$ robots, or agents, with positions denoted by $\textbf{p}_i(t)\in\mathbb{R}^3$, with $i\in\{1,\dots,N\}$. Agents are able to measure their relative distance to a subset of the other agents in a bidirectional way, i.e., with both agents calculating a common ranging estimation simultaneously. The set of robots and estimated distances between them are modeled by a graph $\mathcal{G}=(\mathcal{V},\mathcal{E})$, where $\{1,\dots,N\}$ is a set of $N$ vertices and $\mathcal{E} \subset \mathcal{V}\times \mathcal{V}$ is a set of $M \leq N(N-1)/2$ edges. We consider undirected graphs, i.e., $(i,j) \in \mathcal{E} \Longleftrightarrow (j,i) \in \mathcal{E}$. It is worth noting that the graph does not need to be fully connected, and only a subset of ranging measurements are needed.

We consider robots in three-dimensional space. Nonetheless, for the purpose of collaborative localization, and without a loss of generality, we assume that the position of each agent is given by $\textbf{p}_i\in\mathbb{R}^2$. Even if a locally rigid graph is achieved~\cite{queralta2020uwb}, leading to a single solution to the relative localization problem (i.e., a single localization graph realization), the null space of the transformations is defined by rototranslations of the graph realization in $\mathbb{R}^2$. 

We model UWB range measurements with Gaussian noise:
\begin{equation}
    \textbf{z}^{UWB}_{(i,j),\:(i,j)\in\mathcal{E}} = \lVert \textbf{p}_i(t)-\textbf{p}_j(t) \lVert + \mathcal{N}(0,\sigma_{UWB})
\end{equation}
where $\sigma_{UWB}$ is obtained experimentally from our previous works~\cite{almansa2020autocalibration, torrico2023benchmarking}.

Odometry egomotion estimations for each of the robots are modeled with
\begin{dmath}
    \textbf{z}^{odom}_{i,\:i\in\mathcal{V}} = \left[ \begin{array}{cc} \textbf{R}_i(t-\delta t)\hat{\textbf{R}}_i(t) & \lVert \textbf{p}_i(t)-\textbf{p}_i(t-\delta t) \lVert \\ 0 & 1 \end{array} \right] + \mathcal{N}(0,\:\sigma_{odom})
\end{dmath}
where we utilize $\sigma_{odom} < \sigma_{UWB}/10$, validated experimentally, and $\delta t$ is the output frequency of the Turtlebot's odometry, $\textbf{R}_i(t)$ is the orientation matrix for agent $i$ and $\hat{\textbf{R}}_i(t)$ the relative egomotion estimation in the interval $(t-\delta t, t]$. In practice, we generate the distribution based on the actual covariance matrix given by the odometry estimations themselves.

Finally, when robots are able to detect the same object simultaneously, we also consider these cooperative spatial detection measurements modeled by
\begin{dmath}
    \textbf{z}^{det}_{(i,j),\:(i,j)\in\mathcal{E}} = \textbf{rp}_{i,j} + \mathcal{N}\left((0,0),(\sigma_{det},\sigma_{det})\right) \\ { \text{if} \:\: \lVert \textbf{rp}_{i,j} \rVert < d^{det}_{th} \:\:\: \text{with} } \\
    { \textbf{rp}_{i,j} = \left( \textbf{q}_i^{obj_{k_i}}(t) - \textbf{p}_i(t) \right) - \left(\textbf{q}_j^{obj_{k_j}}(t) - \textbf{p}_j(t) \right) }
\end{dmath}
where we estimate a full relative position estimation $\textbf{rp}_{i,j} \in \mathbb{R}^2$, given object detections $det_{k_i}$ and $def_{j_j}$ and object positions $\textbf{q}_i^{obj_{k_i}}(t)$ and $\textbf{q}_j^{obj_{k_j}}(t)$ relative to robots $i$ and $j$ local reference frames, respectively. To validate that the same object is being used, we use a distance threshold $d^{det}_{th}$.

We consider a system of \(n\) robots, with corresponding inter-robot UWB ranges denoted as \(\mathcal{R}_{p_{i,j}}^t, i,j  \in (1 \sim n)\) at the time \(t\) where \(p_{i,j}\) indicates the pair of UWB transceivers. 

Prior to the PF process, an LSTM model was trained and employed to estimate the ranging error between each UWB pair. The details of this part can be found in section~\ref{lstm-estimation}.

\subsection{Optimization Problem Formulation}

% $x^{(i)}_{\text{pred}} \sim p(x^{(i)}|x^{(i-1)})$
% \red{As demonstrated in the following experiment, LSTM inference can be performed in real-time. We directly integrated this process at the point of reception of the UWB ranges. The efficacy of the LSTM model was evaluated through experiments, demonstrating its capability for real-time inference. }
% The states of the filter are noted as \(S_i = \{x_i, y_i \}, i \in n\). 

The probability density function (pdf) indicating the importance density denoted as \(p(S_t^k | S_{t-1}^k)\) in the particle filter is modeled as a Gaussian distribution as given in Eq.~(\ref{equ:particle})
% p(S_{0:t} | z_{1:t}) \approx \sum_{i=1}^{N_s} \omega_t^i\delta(S_{0:t} - S_{0:t}^i) 

\begin{equation}\label{equ:particle}
\begin{aligned}
    S^k(t) &\sim \mathcal{N}(S_{t-1}^k + \textbf{z}^{odom}_{i}(t), \mathcal{Q}_i(t)), k \in 1 \sim N_s
    % &\approx \sum_{i=1}^{N_s} \omega_t^i\delta(S_{0:t} - S_{0:t}^i)
\end{aligned}
\end{equation}

\noindent where global state $S_k$ at time $t$ is predicted based on a sample drawn from a Gaussian distribution with a mean vector \(S_{t-1}^k + \textbf{z}^{odom}_{i}(t)\) and covariance matrix \(\mathcal{Q}_i(t)\). 

\noindent\textit{b) Weight calculation}: we can now calculate the normalized weights based on a proportional ratio to the importance density probability:

% \(u_{fwd}\), \(u_{ang}\)

% \begin{equation}
%     \begin{bmatrix}
%         z_{dist} \\
%         z_{ang}
%     \end{bmatrix}_k 
%     = 
%     \begin{matrix}
%         \sqrt{(x_{r,k} - x_{lm})^2 + (y_{r,k} - y_{lm})^2} \\
%         \arctan(\frac{y_{r,k} - y_{lm}}{x_{r,k} - x_{lm}})
%     \end{matrix}
% \end{equation}

\begin{equation}
    \omega^k(t) \propto \omega_^k(t-1) p \left(x^k(t-1) | x_^k(t-1) \right)
\end{equation}

\noindent where $\omega^k(t)$ and $x^k(t)$ are the weight and state for particle $k$ at time $t$, respectively.


% \begin{equation}
%     \begin{bmatrix}
%         \widehat{z}_{dist}^k \\
%         \widehat{z}_{ang}^k
%     \end{bmatrix}_t^j
% \end{equation}

% \begin{equation}
%     p(x_t^k | x_{t-1}^k) = \prod_{j=1}^{4} \mathcal{N} (
%     \begin{bmatrix}
%         \widehat{z}_{dist}^k \\
%         \widehat{z}_{ang}^k
%     \end{bmatrix}_t^j
%     ;
%     \begin{bmatrix}
%         z_{dist}^k \\
%         z_{ang}^k
%     \end{bmatrix}_t^j
%     ,
%     R
%     )
% \end{equation}


% Here \(\{ \omega_t^i, S_{0:t}^i\}_{i=1}^{N_s}\) is a set containing \(N_s\) samples and weights. \(\omega_t^i\) denotes the relative importance of each of the \(N_s\) samples \(S_{0:t}^i\) and \(\sum_{i=1}^{N_s} \omega_t^i = 1\). \(\delta(.)\) represents the Dirac delta function. The  \(\delta(a)\) is zero everywhere except for \(a\). 
The iterative particle filter updates are as follows: %process into the following steps:




\noindent\textit{a) Initialization:} We initialize the states of \(M\) particle samples, \(S^{t} = \{ s^t_k\}, k \in M \) based on the odometry data \(O_i^t = \{x_i, y_i\}_t, i \in (1, \dots, N)\) from each robot  at time \(t\) in a Gaussian-distributed manner in Eq.(~\ref{equ:gaussion}) where \( \sigma = 0.2m \) in our experiment.  
\begin{equation}\label{equ:gaussion}
    p(S_{t=0}^k) = \frac{1}{{\sigma \sqrt {2\pi } }}e^{{{ - \left( {O_i^t} \right)^2 } \mathord{\left/ {\vphantom {{ - \left( {x - \mu } \right)^2 } {2\sigma ^2 }}} \right. \kern-\nulldelimiterspace} {2\sigma ^2 }}}
\end{equation}
with associated weights:
\begin{equation}\label{equ:weights}
     w_{t=0}^{i} = \frac{1}{N_s}, i \in 0 \sim n
\end{equation}

% \item Prediction
\noindent\textit{b) Prediction:} We then propagate particles forward using a motion model based on the translation from odometry data:
% \begin{equation}
%     x_t^k \sim \mathcal{N}(x_{t-1}^k + B_tu_t, \mathcal{Q})
% \end{equation}
% \begin{equation}
%     \begin{aligned}
%     \underbrace{
%             \begin{bmatrix}
%                 x_r\\
%                 y_r\\
%                 \theta_r
%             \end{bmatrix}_t 
%         }_{S_{pred}^t} = 
%     \underbrace{
%         \begin{bmatrix}
%             x_r\\
%             y_r\\
%             \theta_r
%         \end{bmatrix}_{t-1} 
%     }_{S_{t-1}}
%         +
%     \underbrace{
%         \begin{bmatrix}
%             \cos(\theta_r, t-1) & 0 \\
%             \sin(\theta_r, t-1) & 0 \\
%             0   & 1 \\
%         \end{bmatrix}
%     }_{B_k}
%     \underbrace{
%         \begin{bmatrix}
%             u_{fwd}\\
%             u_{ang}
%         \end{bmatrix}
%     }_{u_k}
%     \end{aligned}
% \end{equation}

% \begin{equation}
%     \begin{aligned}
%     \underbrace{
%             \begin{bmatrix}
%                 x_r\\
%                 y_r\\
%                 \theta_r
%             \end{bmatrix}_t 
%         }_{x_k} = 
%     \underbrace{
%         \begin{bmatrix}
%             x_r\\
%             y_r\\
%             \theta_r
%         \end{bmatrix}_{t-1} 
%     }_{x_{t-1}}
%         +
%     \underbrace{
%         \begin{bmatrix}
%             \cos(\theta_r, t-1) & 0 \\
%             \sin(\theta_r, t-1) & 0 \\
%             0   & 1 \\
%         \end{bmatrix}
%     }_{B_k}
%     \underbrace{
%         \begin{bmatrix}
%             u_{fwd}\\
%             u_{ang}
%         \end{bmatrix}
%     }_{u_k}
%     \end{aligned}
% \end{equation}

\begin{equation}\label{equ:dynamic}
\begin{aligned}
        u_{i}^t 
        &= (x_u, y_u)^t \\
        &= \{u_i^t\}_k \\
        &= \{O_i^t - O_i^{t-1} + v_i^t\}_k, k \in 1 \sim N_s, i \in 1 \sim n\
\end{aligned}
\end{equation}



% \(S_{pred}^t = \{s_{k,pred}^t\} = \{O_i^t - O_i^{t-1}\}_k, k \in 1 \sim M, i \in 1 \sim n\) 
% where \(v_k^t\)  denotes the noise added to the motion model.
% and sample particles from the proposal distribution:
% \begin{equation}
%     x^{(k)}_{\text{pred}} = p(S^{k}|S^{k-1}), k \in 0 \sim N_s
% \end{equation}

% \item Update (Correction)
\paragraph{Update (Correction)}
The observation data \(y\) can be ranged between robots from the UWB pairs or together from the spatial detections.

\begin{equation}
    y = \begin{cases}
    \{UR_{p_{i,j}}^t\} \\
    \{ UR_{p_{i,j}}^t, SD_{cp}\}
    \end{cases}
\end{equation}

so 
\begin{equation}
    [\widehat{z}_{dist}]_t^k = [\sqrt{u_i - u_j}]_{p_{i,j}} 
\end{equation}

\begin{equation}
    [z_{dist}]_t^k = y_t^k, k \in 0 \sim N_s
\end{equation}

Assuming we have \(M\) of observation data, the importance weights for each particle are computed based on the likelihood of the observed data \(y\):
\begin{equation}
  p(y_t|S_t) = \prod_{j = 1}^{M} \mathcal{N}([\widehat{z}_{dist}]_t^k; [z_{dist}]_t^k, \mathcal{R}), k \in 0 \sim N_s
\end{equation}

Simply put, the highest possibility in the above Gaussian distribution is at the location where the expected measurements \([z_{dist}]_t^k\) coincides with the actual measurements \([\widehat{z}_{dist}]_t^k\). \(\mathcal{R}\) represents the measurement noise covariance. 
Based on the Eq.(~\ref{equ:particle}), we propagate the particles.  After this, we normalize the likelihood of obtaining weights:
% \begin{equation}\label{equ:propagation}
% \begin{aligned}
%         p(y|S_{k-1}^t) 
%         &= \{u_i^t\}_k \\
%         &= \{O_i^t - O_i^{t-1} + v_i^t\}_k, k \in 1 \sim N_s, i \in 1 \sim n\
% \end{aligned}
% \end{equation}
% \begin{equation}
%     w^{(k)} = \frac{p(y|x^{(k)}_{\text{pred}})}{\sum_{k=1}^{N} p(y|x^{(k)}_{\text{pred}})}, k \in 0 \sim N_s
% \end{equation}
\begin{equation}
    w^{k}_t  \propto w^{k}_{t-1} p(y_t | S_t)
\end{equation}

% \item Resampling
\paragraph{Resampling}

Perform resampling to obtain a new set of particles based on their weights as probabilities.

% \item Estimation
\paragraph{Estimation}

Calculate the estimate of the states based on the weighted average of the particles. The estimated state $S_t$ is given by:
\begin{equation}
    S_{t} = \sum_{i=1}^{N_s} w^{(i)} \cdot S^{(i)}
\end{equation}


% \item Repeat
% \paragraph{Repeat}

% Repeat Steps b) to e) for each new measurement or time step to update the state estimate, iteratively.

% \end{enumerate}

% \red{After the initialization, the PF incorporates the UWB ranges from all pairs of UWB transceivers between the robots as the input of the PF. Additionally, as the robots continuously carry out the spatial detections, we compare each pair of detections from each robot and calculate the relative pose between two robots detecting the same object. We then utilize the relative pose of the robot pair calculated via spatial detection as an additional input of PF, whenever available. In the determination of  the spatial detection from the same object obtained by two robots, we compared the relative range calculated based on the spatial detection with the UWB range among the robots. Only ranges within a threshold of the UWB range are accepted and identified as measurements obtained from an object in both robots' fields of view. }


% if it is similar, then it is the same object.


% Prior to the Particle Filter (PF) process, a Long Short-Term Memory (LSTM) model was employed to estimate the ranging error between each Ultra-Wideband (UWB) pair. 
% The efficacy of the LSTM model was evaluated through experiments, demonstrating its capability for real-time inference. 
% This estimation process was directly integrated at the point of receipt of the UWB ranges.

% The PF process was initiated by initializing the particles using odometry data obtained from each robot, in a Gaussian distribution. The UWB ranges from all pairs of UWB tags among the Turtlebot4 robots were then incorporated as inputs to the PF. Additionally, as the robots continuously performed spatial detections, relative poses between pairs of robots detecting the same object were calculated and utilized as inputs to the PF, once they were determined through comparison of each pair of detections.


\subsection{LSTM network for UWB ranging error estimation}\label{lstm-estimation}
% \subsubsection{Variants of LSTM}

In this study, we utilized three variants of LSTM networks. The specific variants are (i) stacked LSTM, (ii) bidirectional LSTM, and (iii) convLSTM. These models were trained separately for each UWB pair.
The inputs of these networks are the UWB range of the UWB pair, $UR$, and the two orientations of robots, $OR0$ and $OR1$, where the UWB pair is equipped. Details about the applied LSTM network information can be seen in Figure~\ref{fig:lstms}. 
% \begin{figure}[h]
%     \centering
%     \begin{subfigure}{.16\textwidth}
%         \includegraphics[width=\textwidth]{fig/lstm.png}
%         \caption{LSTM}
%         \label{fig:stackedlstm}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{.14\textwidth}
%         \includegraphics[width=0.88\textwidth]{fig/bilstm.png}
%         \caption{Bi LSTM}
%         \label{fig:bilstm}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{.15\textwidth}
%         \includegraphics[width=\textwidth]{fig/convlstm.png}
%         \caption{convLSTM}
%         \label{fig:conv_lstm}
%     \end{subfigure}
%     \caption{The layer details of LSTM variants applied in this experiment. $UR$ is the UWB range, $OR0$ is the orientation of one robot while $OR1$ is of the other robot.}
%     \label{fig:lstms}
% \end{figure}

\begin{figure}[t]
    \centering
    % \includegraphics[width=0.45\textwidth]{fig/lstm_01.pdf}
    \includegraphics[width=0.45\textwidth]{fig/lstm-new.pdf}
    \caption{The layer details of LSTM variants applied in this experiment. $UR$ is the UWB range, $OR0$ is the orientation of one robot and $OR1$ is from the other robot in the robot pair.}
    \label{fig:lstms}
\end{figure}

For estimating the current UWB ranging error, the LSTM takes $n\_steps$ frames of the data $[\, UR, OR0, OR1 ] \,$ as the input. The output of the dense layer at the end of the LSTM network is then a single UWB ranging error. % is obtained as the output.
% And the output is obtained by a dense layer with only one number as the output.
% We trained the models based on the data we collected for each UWB pair.

The individual LSTM networks are trained using data from a separate experiment using the same robots in the same location. Therefore, we expect the networks to be able to model antenna delays and predict potential errors based on the relative orientation of the antennas. This limits the generalization of the results, but we do separate in time the training data from the final experiments reported in this paper.




\subsection{Hardware information}

The mobile robot platforms used in the experiments are five Turtlebot4 Lite %~\cite{turtlebot4} 
robots, denoted $\mathcal{R}_{i,\:i\in\{0,1,2,3,4\}}$. We use these robots for both data collection and real-world navigation based on our proposed UWB-based relative estate estimation method. Figure~\ref{fig:harware_00}\,(b) shows the customized Turtlebot4 platform where we equip a Qorvo DWM1001 UWB transceiver%~\cite{uwb-dev} 
and an OAK-D stereo camera (replacing the default OAK-D Lite).%~\cite{oak-d-lite} are equipped. 
We run all our code in a Jetson Nano computer, to which the OAK-D camera is connected. The Turtlebot4 ROS\,2 drivers run on the existing Raspberry 4.
% The UWB can achieve centimeter-level out-of-box ranging accuracy. 
The UWB transceivers in this experiment were programmed to iteratively measure the time of flight (ToF) between pairs to obtain ranging measurements. The OAK-D stereo cameras provide poses of the detected objects relative to the cameras. The odometry measurements are given directly by the Turthebot4 ROS\,2 driver. %Regarding the odometry information which has been utilized in our proposed PF approach, the Turtlebot4 has its own IMU providing highly accurate built-in odometry information.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{fig/4xtbots_uwb_experiment.pdf}
    \caption{Experimental site and platforms. Subfigure (a) shows the motion capture (MOCAP) arena and the moving patterns of four Turtlebot4 robots. Subfigure (b) shows the customized Turtlebot4 platform mounted with a single UWB transceiver, an OAK-D stereo camera, and a Jetson Nano.}
    \label{fig:harware_00}
\end{figure}

The experimental site is shown in figure~\ref{fig:harware_00}(a); the robots navigate within an arena with an OptiTrack motion capture system providing the ground truth to verify the estimated relative states of each robot. 
% The experimental site can be seen in Figure~\ref{fig:harware_00}(a). 
The operating area is approx. $8\,m\times9\,m\times5\,m$. Inside the area, we place a static robot $\mathcal{R}_{4}$ and four moving robots $\mathcal{R}_{i,\:i\in\{0,1,2,3\}}$. The former serves to align references while the latter four follow the paths shown in figure~\ref{fig:harware_00}(a) of a triangle, a $X$, a circle, and a rectangle, respectively. It is worth mentioning that the origin of coordinate $XO_2Y$ is the $(0,0)$ of the MOCAP system while the origin of coordinate $XO_1Y$ is the static robot $\mathcal{R}_{4}$ we set as the origin of the robots' relative positions. We assume that robots have a common orientation frame (e.g., through a compass) to allow for single-range relative state estimation.

In terms of the objects for the robots to obtain spatial detection, several selected objects including bottles, chairs, and cups are arbitrarily placed inside and outside the experimental site. A pretrained YOLOv4 network is used, allowing for any COCO object to be used for cooperative spatial detections.

\subsection{Multi-robot relative localization system implementation}

Our system was built on the basis of ROS\,2 for communication among robots. 
We deployed ROS\,2 with Zenoh for the scalability of the multi-robot system as Zenoh significantly reduced the communication cost, while DDS remained the internal middleware within each of the individual robots. 
In ROS\,2, the primary approach to communicating is to send messages in the form of topics. The Turtlebot4 works originally with ROS\,2 and has a comprehensive ecosystem. The topics and other services have the same names for each robot. For differentiating the robots in the communication of the multi-robot system, the original ROS\,2 can work by providing different namespaces. Adding the namespace, however, requires many modifications to Turtlebot4's software to make everything work including the ROS\,2 navigation stack. It is challenging to make them communicate efficiently while keeping the robots as original as they were. Our solution is to deploy Zenoh with ROS\,2. The details can be seen in figure~\ref{fig:ros_zenoh_diagram}. In the system, we have the robots, the Zenoh Router, and the engine for localization and control. The engine for localization and control is either a computer or any Raspberry Pi or Jetson Nano from the robots. In our case, we deployed it on our own laptop, but we show that the computational resources of either embedded computer suffices. On the robot side, as all the topics across the robots are the same, we deployed the Zenoh clients with different $ZENOH\_SCOPE$ for each robot without changing any other settings within the robot (common DDS domain id and topic names across robots). We then hosted a Zenoh router for discovering and transferring messages of the topics through the Zenoh DDS bridge~\footnote{\url{https://github.com/eclipse-zenoh/zenoh-plugin-dds}} to the engine for localization and control, where we receive the ground truth from the MOCAP system as well.  Each scope is mapped to a different domain id at the controller end, with the DDS domain bridge merging these with topic namespacing~\footnote{\url{https://github.com/ros2/domain\_bridge}}. It is worth mentioning that the topic names are also the same in the receiving end, which is the engine, so we can simplify the localization and control process. %So we have the DDS domain bridge~\footnote{\url{https://github.com/ros2/domain\_bridge}}     to distinguish the topics by domain IDs for different robots. 
We can take the odometry topic as an example. Within the robots, it is $\backslash odom$. However, in the Zenoh communication network, the topic names  will be $\backslash\text{tb}\{i\}\backslash odom$ (where $\backslash\text{tb}\{i\}$ is the Zenoh scope). In the localization engine, the topic names will be $\backslash odom$ with different domain IDs, or again $\backslash\text{tb}\{i\}\backslash odom$ at the common domain id (with $\backslash\text{tb}\{i\}$ now acting as a ROS topic namespace).
Our core code for the particle filter localization is based on the pfilter library\footnote{\url{https://github.com/johnhw/pfilter}}%~\cite{pfilter} 
and we rewrote parts of it to suit our program. %The details of our codes can be seen in our GitHub\footnote{\url{https://github.com/TIERS/uwb\_mrs}}. 
For LSTM-based UWB ranging error estimation, we applied TensorFlow Keras to build our own model and performed the training and real-world inference.
% And TensorFlow Keras was used for the learning of UWB ranging error. \red{More content here}

\input{algs/pf_relative}

\begin{figure}[t]
    \centering
    \includegraphics[width=.49\textwidth]{fig/ros_zenoh_diagram.pdf}
    \caption{Implementation of the System with ROS\,2 and Zenoh}
    \label{fig:ros_zenoh_diagram}
\end{figure}


% \subsubsection{Setting}
% \subsection{Experimental Setup}
% In the experiment, two robots kept static and the other three robots did three different patterns: circle, rectangle, and zigzag path, repeatedly. Based on the turtlebot4 navigation stack, we designed the waypoints in the made occupancy map ahead as shown below in figure~\ref{fig:moving_data}.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.45\textwidth]{fig/robots_arena.png}
%     \caption{Robot Moving Patterns for the data collection in our experiment}
%     \label{fig:moving_data}
% \end{figure}
% \subsection{Data Collection}
% \subsection{UWB Range Error Fit}




\subsection{Evaluation on multiple mobile computing platforms}

As there are multiple popular computing platforms for multi-robot systems nowadays, it is valuable to provide a performance evaluation of the proposed approach as a reference for research in the field. We evaluated the memory consumption and the computation time on platforms including an Intel computer, an NVIDIA Jetson Nano, and a Raspberry Pi 4B in Turtlebot4. The Intel computer has 32\,GB of DDR4 RAM memory while the Jetson Nano and Raspberry Pi 4B have 4\,GB RAM memory. We run the PF code without the LSTM for the UWB ranging error correction as it requires GPU support. More detailed specifications of the computing platforms can be found in Table~\ref{tb:computing}. In our experiments, the Jetson Nano is needed for both spatial detections and LSTM deployment. However, the majority of the computation regarding spatial detection (both the YOLO detector and the depth data fusion) is done onboard the OAK-D camera on the robots and does not need a GPU in the companion computer.

\begin{table}[b]
    \caption{Specifications of the computing platforms.}
    \resizebox{0.49\textwidth}{!}{
        \begin{tabular}{ccc}
            \toprule[0.3mm]
            \textbf{Computing Platform} & \textbf{PROCESSOR}                            & \textbf{Memory (GB)} \\ \midrule[0.3mm]
            \textbf{Intel PC}                    & 11th Gen Intel(R) Core(TM) i9-11900H @ 2.5GHZ & 32                   \\ 
            \textbf{Jetson Nano}                 & Quad-core ARM Cortex-A57 64-bit @ 1.43 GH     & 4                    \\ 
            \textbf{Raspberry Pi 4B}             & Quad-core  ARM Cortex-A72 64-bit @ 1.5 GHz    & 4                    \\ \toprule[0.3mm]
        \end{tabular}
    }
    \label{tb:computing}
\end{table}

% The detailed specification of these platforms are shown in the table below.

\subsection{Navigation based on proposed relative state estimation}

To validate the relative state estimated by our PF approach we estimate both positioning and navigation errors. For the positioning error, the robots follow trajectories using the MOCAP data as feedback for the controller. In the autonomous navigation part, we set one robot performing a navigation task in the shape of a rectangle using the aforementioned relative position method for the controller feedback.
% In the navigation part, based on the relative positioning approach, the robot performed the navigation. 

==> tex/lstm/lstm_mse.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{gainsboro229}{RGB}{229,229,229}
\definecolor{lightblue}{RGB}{173,216,230}
\definecolor{lightgray}{RGB}{211,211,211}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{lightgreen}{RGB}{144,238,144}
\definecolor{pink}{RGB}{255,192,203}

% \definecolor{color0}{rgb}{0.1,0.1,0.1}
% % \definecolor{color1}{rgb}{1,0.752941176470588,0.796078431372549}
% % \definecolor{color2}{rgb}{0.67843137254902,0.847058823529412,0.901960784313726}
% % \definecolor{color3}{rgb}{0.501960784313725,0,0.501960784313725}
% % \definecolor{color4}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
% \definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
% \definecolor{color2}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
% \definecolor{color3}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
% \definecolor{color4}{rgb}{0.890196078431372,0.466666666666667,0.76078431372549}

\definecolor{color0}{rgb}{0.90, 0.62, 0.00}
\definecolor{color1}{rgb}{0.34, 0.70, 0.91}
\definecolor{color2}{rgb}{0.00, 0.62, 0.45}
\definecolor{color3}{rgb}{0.94, 0.89, 0.27}
\definecolor{color4}{rgb}{0.00, 0.45, 0.69}
\definecolor{color5}{rgb}{0.83, 0.37, 0.00}



\begin{axis}[
    height=\figureheight,
    width=\figurewidth,
    % legend cell align={left},
    % legend style={
    %   fill opacity=0.8,
    %   draw opacity=1,
    %   text opacity=1,
    %   at={(0.9,0.5)},
    %   anchor=west,
    %   draw=white!80!black
    % },
    axis line style={white},
    % tick align=outside,
    % tick pos=left,
    x grid style={white!69.0196078431373!black},
    % xtick style={color=black},
    % y grid style={white!90!black},
    % ymajorgrids,
    % ytick style={color=black},
    % scaled y ticks = false,
% axis background/.style={fill=lightgray},
% legend cell align={left},
% legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
% x grid style={darkgray176},
xmin=0, xmax=3.5,
xtick style={color=black},
xtick={1,2,3},
% xticklabel style={rotate=45},
xticklabels={$SL$,$BL$,$CL$},
y grid style={gainsboro229},
ylabel={MSE ($m^2$)},
    minor y tick num = 4,
    minor y grid style={dashed},
    ymajorgrids,
    ymajorgrids=true,
    ymajorticks=true,
ymin=0.00201161395, ymax=0.02124389295,
    yminorgrids,
    yminorgrids=true,
ytick style={color=black}
]
\path [draw=color0, fill=color0, opacity=0.5]
(axis cs:0.75,0.006506678)
--(axis cs:1.25,0.006506678)
--(axis cs:1.25,0.016034873)
--(axis cs:0.75,0.016034873)
--(axis cs:0.75,0.006506678)
--cycle;
\addplot [color0, forget plot]
table {%
1 0.006506678
1 0.0043022274
};
\addplot [color0, forget plot]
table {%
1 0.016034873
1 0.020232279
};
\addplot [color0, forget plot]
table {%
0.875 0.0043022274
1.125 0.0043022274
};
\addplot [color0, forget plot]
table {%
0.875 0.020232279
1.125 0.020232279
};
\path [draw=color0, fill=color0, opacity=0.5]
(axis cs:1.75,0.00591682)
--(axis cs:2.25,0.00591682)
--(axis cs:2.25,0.012127121)
--(axis cs:1.75,0.012127121)
--(axis cs:1.75,0.00591682)
--cycle;
\addplot [color0, forget plot]
table {%
2 0.00591682
2 0.0039952816
};
\addplot [color0, forget plot]
table {%
2 0.012127121
2 0.014664161
};
\addplot [color0, forget plot]
table {%
1.875 0.0039952816
2.125 0.0039952816
};
\addplot [color0, forget plot]
table {%
1.875 0.014664161
2.125 0.014664161
};
\path [draw=color0, fill=color0, opacity=0.5]
(axis cs:2.75,0.0052745285)
--(axis cs:3.25,0.0052745285)
--(axis cs:3.25,0.0110784575)
--(axis cs:2.75,0.0110784575)
--(axis cs:2.75,0.0052745285)
--cycle;
\addplot [color0, forget plot]
table {%
3 0.0052745285
3 0.0031587675
};
\addplot [color0, forget plot]
table {%
3 0.0110784575
3 0.011096034
};
\addplot [color0, forget plot]
table {%
2.875 0.0031587675
3.125 0.0031587675
};
\addplot [color0, forget plot]
table {%
2.875 0.011096034
3.125 0.011096034
};
% \addplot [semithick, pink]
% table {%
% 0 0
% 1 0
% };
% \addlegendentry{stacked_lstm}
% \addplot [semithick, lightblue]
% table {%
% 0 0
% 1 0
% };
% \addlegendentry{bidirectional_lstm}
% \addplot [semithick, color3]
% table {%
% 0 0
% 1 0
% };
% \addlegendentry{convlstm}
\addplot [thick, white, forget plot]
table {%
0.75 0.010918155
1.25 0.010918155
};
\addplot [thick, white, forget plot]
table {%
1.75 0.008036631
2.25 0.008036631
};
\addplot [thick, white, forget plot]
table {%
2.75 0.0075195907
3.25 0.0075195907
};
\end{axis}

\end{tikzpicture}


==> tex/lstm/lstm_time.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{gainsboro229}{RGB}{229,229,229}
\definecolor{lightblue}{RGB}{173,216,230}
\definecolor{lightgray}{RGB}{211,211,211}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{lightgreen}{RGB}{144,238,144}
\definecolor{pink}{RGB}{255,192,203}

\definecolor{color0}{rgb}{0.1,0.1,0.1}
% \definecolor{color1}{rgb}{1,0.752941176470588,0.796078431372549}
% \definecolor{color2}{rgb}{0.67843137254902,0.847058823529412,0.901960784313726}
% \definecolor{color2}{rgb}{0.501960784313725,0,0.501960784313725}
% \definecolor{color4}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color2}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color3}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color4}{rgb}{0.890196078431372,0.466666666666667,0.76078431372549}

\definecolor{color0}{rgb}{0.90, 0.62, 0.00}
\definecolor{color1}{rgb}{0.34, 0.70, 0.91}
\definecolor{color2}{rgb}{0.00, 0.62, 0.45}
\definecolor{color3}{rgb}{0.94, 0.89, 0.27}
\definecolor{color4}{rgb}{0.00, 0.45, 0.69}
\definecolor{color5}{rgb}{0.83, 0.37, 0.00}


\begin{axis}[
    height=\figureheight,
    width=\figurewidth,
    % legend cell align={left},
    % legend style={
    %   fill opacity=0.8,
    %   draw opacity=1,
    %   text opacity=1,
    %   at={(0.9,0.5)},
    %   anchor=west,
    %   draw=white!80!black
    % },
    axis line style={white},
    % tick align=outside,
    % tick pos=left,
    x grid style={white!69.0196078431373!black},
    % xtick style={color=black},
    % y grid style={white!90!black},
    % ymajorgrids,
    % ytick style={color=black},
    % scaled y ticks = false,
% axis background/.style={fill=lightgray},
% legend cell align={left},
% legend style={
%   fill opacity=0.8,
%   draw opacity=1,
%   text opacity=1,
%   at={(0.03,0.97)},
%   anchor=north west,
%   draw=lightgray204
% },
tick align=outside,
tick pos=left,
% x grid style={darkgray176},
xmin=0, xmax=3.5,
xtick style={color=black},
xtick={1,2,3},
% xticklabel style={rotate=45},
xticklabels={$SL$,$BL$,$CL$},
y grid style={gainsboro229},
ylabel={Computation Time (S)},
    minor y tick num = 4,
    minor y grid style={dashed},
    ymajorgrids,
    ymajorgrids=true,
    ymajorticks=true,
ymin=0.025, ymax=0.0933806419372558,
    yminorgrids,
    yminorgrids=true,
% ytick style={color=black}
]
\path [draw=color1, fill=color1, opacity=0.5]
(axis cs:0.75,0.0395587682723998)
--(axis cs:1.25,0.0395587682723998)
--(axis cs:1.25,0.0446183681488037)
--(axis cs:0.75,0.0446183681488037)
--(axis cs:0.75,0.0395587682723998)
--cycle;
\addplot [color1, forget plot]
table {%
1 0.0395587682723998
1 0.0390398502349853
};
\addplot [color1, forget plot]
table {%
1 0.0446183681488037
1 0.0471384525299072
};
\addplot [color1, forget plot]
table {%
0.875 0.0390398502349853
1.125 0.0390398502349853
};
\addplot [color1, forget plot]
table {%
0.875 0.0471384525299072
1.125 0.0471384525299072
};
\path [draw=color1, fill=color1, opacity=0.5]
(axis cs:1.75,0.0353068113327026)
--(axis cs:2.25,0.0353068113327026)
--(axis cs:2.25,0.0460824966430664)
--(axis cs:1.75,0.0460824966430664)
--(axis cs:1.75,0.0353068113327026)
--cycle;
\addplot [color1, forget plot]
table {%
2 0.0353068113327026
2 0.029287576675415
};
\addplot [color1, forget plot]
table {%
2 0.0460824966430664
2 0.0546913146972656
};
\addplot [color1, forget plot]
table {%
1.875 0.029287576675415
2.125 0.029287576675415
};
\addplot [color1, forget plot]
table {%
1.875 0.0546913146972656
2.125 0.0546913146972656
};
\path [draw=color1, fill=color1, opacity=0.5]
(axis cs:2.75,0.0659770965576172)
--(axis cs:3.25,0.0659770965576172)
--(axis cs:3.25,0.0853276252746582)
--(axis cs:2.75,0.0853276252746582)
--(axis cs:2.75,0.0659770965576172)
--cycle;
\addplot [color1, forget plot]
table {%
3 0.0659770965576172
3 0.0625183582305908
};
\addplot [color1, forget plot]
table {%
3 0.0853276252746582
3 0.0889339447021484
};
\addplot [color1, forget plot]
table {%
2.875 0.0625183582305908
3.125 0.0625183582305908
};
\addplot [color1, forget plot]
table {%
2.875 0.0889339447021484
3.125 0.0889339447021484
};
% \addplot [semithick, pink]
% table {%
% 0 0
% 1 0
% };
% % \addlegendentry{stacked_lstm}
% \addplot [semithick, lightblue]
% table {%
% 0 0
% 1 0
% };
% % \addlegendentry{bidirectional_lstm}
% \addplot [semithick, lightgreen]
% table {%
% 0 0
% 1 0
% };
% \addlegendentry{convlstm}
\addplot [thick, white, forget plot]
table {%
0.75 0.041311502456665
1.25 0.041311502456665
};
\addplot [thick, white, forget plot]
table {%
1.75 0.0381174087524414
2.25 0.0381174087524414
};
\addplot [thick, white, forget plot]
table {%
2.75 0.0701932907104492
3.25 0.0701932907104492
};
\end{axis}

\end{tikzpicture}


==> tex/nav/nav_ape_ate.tex <==
% This file was created with tikzplotlib v0.10.1.
\tikzexternaldisable
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{steelblue31119180}{RGB}{31,119,180}
% \definecolor{color0}{rgb}{0.1,0.1,0.1}
% \definecolor{color1}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
% \definecolor{color2}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
% \definecolor{color3}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
% \definecolor{color4}{rgb}{0.890196078431372,0.466666666666667,0.76078431372549}

\definecolor{color0}{rgb}{0.90, 0.62, 0.00}
\definecolor{color1}{rgb}{0.34, 0.70, 0.91}
\definecolor{color2}{rgb}{0.00, 0.62, 0.45}
\definecolor{color3}{rgb}{0.94, 0.89, 0.27}
\definecolor{color4}{rgb}{0.00, 0.45, 0.69}
\definecolor{color5}{rgb}{0.83, 0.37, 0.00}

\begin{axis}[
    height=\figureheight,
    width=\figurewidth,
    axis line style={white},
    tick align=outside,
    tick pos=left,
    % title={State Estimation Error},
    % x grid style={lightgray204},
    % xlabel=\textcolor{black}{Approaches},
    % xmajorgrids,
    % xmajorticks=false,
    xmin=0.5, xmax=2.5,
    % xminorgrids,
    % xtick style={color=darkslategray38},
    xtick={1, 2},
    xticklabels={ATE, APE},
    % y grid style={green},
    ylabel={RMSE (m)},
    minor y tick num = 4,
    minor y grid style={dashed},
    ymajorgrids,
    ymajorgrids=true,
    ymajorticks=true,
    ymin=-0.02, ymax=0.31,
    yminorgrids,
    yminorgrids=true,
    enlarge y limits=.05,
    % ytick style={color=darkslategray38}
]

% \begin{axis}[
% tick align=outside,
% tick pos=left,
% x grid style={darkgray176},
% xmin=0.5, xmax=3.5,
% xtick style={color=black},
% y grid style={darkgray176},
% ymin=-0.0150005148967841, ymax=0.315069674565589,
% ytick style={color=black}
% ]
\addplot [color0]
table {%
1 0.053873981969673
1 2.67553332378156e-06
};
\addplot [color0]
table {%
1 0.188856467646929
1 0.245005847565849
};
\addplot [color0]
table {%
0.875 2.67553332378156e-06
1.125 2.67553332378156e-06
};
\addplot [color0]
table {%
0.875 0.245005847565849
1.125 0.245005847565849
};
\addplot [color1]
table {%
2 0.0466222337255707
2 0.000166469555703272
};
\addplot [color1]
table {%
2 0.181464587602633
2 0.300066484135481
};
\addplot [color1]
table {%
1.875 0.000166469555703272
2.125 0.000166469555703272
};
\addplot [color1]
table {%
1.875 0.300066484135481
2.125 0.300066484135481
};
\path [draw=color0, fill=color0, opacity=0.5]
(axis cs:0.75,0.053873981969673)
--(axis cs:1.25,0.053873981969673)
--(axis cs:1.25,0.188856467646929)
--(axis cs:0.75,0.188856467646929)
--(axis cs:0.75,0.053873981969673)
--cycle;
\path [draw=color1, fill=color1, opacity=0.5]
(axis cs:1.75,0.0466222337255707)
--(axis cs:2.25,0.0466222337255707)
--(axis cs:2.25,0.181464587602633)
--(axis cs:1.75,0.181464587602633)
--(axis cs:1.75,0.0466222337255707)
--cycle;
\addplot [white]
table {%
0.75 0.109420923795199
1.25 0.109420923795199
};
\addplot [white]
table {%
1.75 0.0871759237969218
2.25 0.0871759237969218
};
\end{axis}

\end{tikzpicture}

